Distributed Differentially Private Ranking Aggregation

Ranking aggregation is commonly adopted in cooperative decision-making to assist in combining multiple rankings into a single representative. To protect the actual ranking of each individual, some privacy-preserving strategies, such as differential privacy, are often used. This, however, does not consider the scenario where the curator, who collects all rankings from individuals, is untrustworthy. This paper proposed a mechanism to solve the above situation using the distribute differential privacy framework. The proposed mechanism collects locally differential private rankings from individuals, then randomly permutes pairwise rankings using a shuffle model to further amplify the privacy protection. The final representative is produced by hierarchical rank aggregation. The mechanism was theoretically analysed and experimentally compared against existing methods, and demonstrated competitive results in both the output accuracy and privacy protection.

==> tex/mod-contact.tex <==
%%==========================================================================================
%
\begin{slide}[toc=,bm=]{Questions?}
\begin{center}
\begin{figure}
    \animategraphics[autoplay, loop, height=0.36\textheight]{5}{./graphics//gif//question//q_}{1}{30}
\end{figure}
\end{center}
\end{slide}
%%
%%==========================================================================================


%%==========================================================================================
% Contact Page
%
\begin{wideslide}[toc=,bm=]{Contact Information}
\centering
\vspace{\stretch{1}}
\twocolumn[
lcolwidth=0.35\linewidth,
rcolwidth=0.65\linewidth
]
{
% \centerline{\includegraphics[scale=.2]{tulip-logo.eps}}
}
{
\vspace{\stretch{1}}

  \twocolumn[lcolwidth=0.5\linewidth,
rcolwidth=0.45\linewidth
]{
\vspace{\stretch{2}}

Associate Professor \textsc{\textbf{Gang Li}}\\
School of Information Technology\\
Deakin University\\
Burwood, Victoria 3125, Australia
}
    {
    %\begin{flushleft}
    \parbox{4cm}{%
        \centering 
        \begin{tikzpicture}
            \clip (0,0) circle (.16\textwidth); %2cm
            \node[anchor=center] at (0,0) %(0.62,-3) 
            {\includegraphics[width=0.33\textwidth]{./graphics/tulip/gangli.eps}};
        \end{tikzpicture}
    } %parbox
%       \includegraphics[width=.36\textwidth]{figures/tulip/gangli.eps}
%     \end{flushleft}
    }

%

\begin{description}
 \item[\textcolor{orange}{\faEnvelope}] \href{mailto:gangli@tulip.org.au}
 {\textsc{\footnotesize{gangli@tulip.org.au}}}

 \item[\textcolor{orange}{\faGithub}] \href{https://github.com/tulip-lab}
 {\textsc{\footnotesize{Open Resources of TULIP-Lab}}}

 \item[\textcolor{orange}{\faHome}] \href{http://www.tulip.org.au}
 {\textsc{\footnotesize{Team for Universal Learning and Intelligent Processing}}}
\end{description}
}

\vspace{\stretch{1}}
\end{wideslide}

==> tex/mod-preamble.tex <==
%
% ---------------------------------------------------------------
% Copyright (C) 2012-2018 Gang Li
% ---------------------------------------------------------------
%
% This work is the default powerdot-tuliplab style test file and may be
% distributed and/or modified under the conditions of the LaTeX Project Public
% License, either version 1.3 of this license or (at your option) any later
% version. The latest version of this license is in
% http://www.latex-project.org/lppl.txt and version 1.3 or later is part of all
% distributions of LaTeX version 2003/12/01 or later.
%
% This work has the LPPL maintenance status "maintained".
%
% This Current Maintainer of this work is Gang Li.
%
%

\usepackage{cancel}
\usepackage{caption}
\usepackage{stackengine}
\usepackage{smartdiagram}
\usepackage{attrib}
\usepackage{amssymb}
\usepackage{amsmath} 
\usepackage{amsthm} 
\usepackage{mathtools}
\usepackage{rotating}
\usepackage{graphicx}
\usepackage{boxedminipage}
\usepackage{rotate}
\usepackage{calc}
\usepackage[absolute]{textpos}
\usepackage{psfrag,overpic}
\usepackage{fouriernc}
\usepackage{pstricks,pst-3d,pst-grad,pstricks-add,pst-text,pst-node,pst-tree}
\usepackage{moreverb,epsfig,subfigure}
\usepackage{color}
\usepackage{booktabs}
\usepackage{etex}
\usepackage{breqn}
\usepackage{multirow}
\usepackage{natbib}
\usepackage{bibentry}
\usepackage{gitinfo2}
\usepackage{siunitx}
\usepackage{nicefrac}
%\usepackage{geometry}
%\geometry{verbose,letterpaper}
\usepackage{media9}
\usepackage{animate}
%\usepackage{movie15}
\usepackage{auto-pst-pdf}

\usepackage{breakurl}
\usepackage{fontawesome}
\usepackage{xcolor}
\usepackage{multicol}



\usepackage{verbatim}
\usepackage[utf8]{inputenc}
\usepackage{dtk-logos}
\usepackage{tikz}
\usepackage{adigraph}
%\usepackage{tkz-graph}
\usepackage{hyperref}
%\usepackage{ulem}
\usepackage{pgfplots}
\usepackage{verbatim}
\usepackage{fontawesome}


\usepackage[linesnumbered,lined,ruled]{algorithm2e}


\usepackage{todonotes}
\usepackage{tablefootnote}
\usepackage{threeparttable}
%\usepackage[numbers]{natbib}
\usepackage{bibentry}
\usepackage{bibunits}

\usepackage[utf8]{inputenc}
\usepackage{dtk-logos}
\usepackage{tikz}
\usetikzlibrary{arrows,chains,mindmap,shadows,automata,patterns,
    petri,shapes.geometric,shapes.misc, spy, trees,decorations.markings}


\usepackage{hyperref}
\hypersetup{ % TODO: PDF meta Data
    pdftitle={TULIP Lab},
    pdfauthor={Gang Li},
    pdfpagemode={FullScreen},
    pdfborder={0 0 0}
}


\usepackage{listings}
\lstset{frameround=fttt, 
frame=trBL, 
stringstyle=\ttfamily,
backgroundcolor=\color{yellow!20},
basicstyle=\footnotesize\ttfamily}
\lstnewenvironment{code}{
\lstset{frame=single,escapeinside=`',
backgroundcolor=\color{yellow!20},
basicstyle=\footnotesize\ttfamily}
}{}



% package to show source code

\definecolor{LightGray}{rgb}{0.9,0.9,0.9}
\newlength{\pixel}\setlength\pixel{0.000714285714\slidewidth}
\setlength{\TPHorizModule}{\slidewidth}
\setlength{\TPVertModule}{\slideheight}
\newcommand\highlight[1]{\fbox{#1}}
\newcommand\icite[1]{{\footnotesize [#1]}}

\newcommand\twotonebox[2]{\fcolorbox{pdcolor2}{pdcolor2}{#1\vphantom{#2}}\fcolorbox{pdcolor2}{white}{#2\vphantom{#1}}}
\newcommand\twotoneboxo[2]{\fcolorbox{pdcolor2}{pdcolor2}{#1}\fcolorbox{pdcolor2}{white}{#2}}
\newcommand\vpspace[1]{\vphantom{\vspace{#1}}}
\newcommand\hpspace[1]{\hphantom{\hspace{#1}}}
\newcommand\COMMENT[1]{}


\newcommand\mx[1]{\begin{math}#1\end{math}}% math expression


\newcommand\placepos[3]{\hbox to\z@{\kern#1
        \raisebox{-#2}[\z@][\z@]{#3}\hss}\ignorespaces} 


%\newtheorem{thm}{Theorem}[chapter] % reset theorem numbering for each chapter

%\usepackage{amsthm}

\newtheorem*{remark}{Remark}
\newtheorem*{theorem}{Theorem}
\newtheorem*{definition}{Definition}
\newtheorem*{proposition}{Proposition}

%\theoremstyle{plain}
%\newtheorem*{theorem}{Theorem}
%\newtheorem*{proposition}[theorem]{Proposition}
%\newtheorem*{definition}[theorem]{Definition}
%\newtheorem*{corollary}[theorem]{Corollary}
%\newtheorem*{lemma}[theorem]{Lemma}

%\theoremstyle{definition}
 % definition numbers are dependent on theorem numbers


%forest
\usepackage{forest}
\usetikzlibrary{arrows.meta, shapes.geometric, calc, shadows}

\colorlet{mygreen}{green!75!black}
\colorlet{col1in}{red!30}
\colorlet{col1out}{red!40}
\colorlet{col2in}{mygreen!40}
\colorlet{col2out}{mygreen!50}
\colorlet{col3in}{blue!30}
\colorlet{col3out}{blue!40}
\colorlet{col4in}{mygreen!20}
\colorlet{col4out}{mygreen!30}
\colorlet{col5in}{blue!10}
\colorlet{col5out}{blue!20}
\colorlet{col6in}{blue!20}
\colorlet{col6out}{blue!30}
\colorlet{col7out}{orange}
\colorlet{col7in}{orange!50}
\colorlet{col8out}{orange!40}
\colorlet{col8in}{orange!20}
\colorlet{linecol}{blue!60}

\definecolor{mynodecolor}{RGB}{198,191,234}

\tikzstyle{flipbox} = [draw=blue!10, fill=green!20, very thick,
rectangle, rounded corners, inner sep=10pt, inner ysep=20pt]
\tikzstyle{fancytitle} =[fill=red, text=white]%, ellipse]
%

%\usepackage{pgfplots}
%\usepackage{tikz}
%%
\usetikzlibrary{positioning, arrows.meta}

\makeatletter
\newcommand\notsotiny{\@setfontsize\notsotiny{7}{8}}
%\newcommand\notsotiny{\@setfontsize\notsotiny\@vipt\@viipt}
\makeatother

==> tex/mod-slides.tex <==
%
% %TODO: This is the place that you need to revise.
%

\section{Background and Motivation}

%=================================================================
%%  
\begin{slide}%[toc=,bm=]
{Targeted Venue}
	\twotonebox{\faHandORight}{\parbox{.96\textwidth}
{  
Select the list of targeted \emph{conferences} and \emph{journals},
based on the \emph{contribution} and 
potential \emph{impact} of the research work~\cite{ZLMLY20J04}
}} 
	
\onslide*{2-3}{
\begin{proof}[Notes]
\begin{itemize}
\item<2-> 
Stick to a small set of \emph{conferences} and \emph{journals}:
	\begin{description}
	\item[Conferences]<2->
	No more than two in each tier:
	\begin{itemize}
	\item AAAI, IJCAI, UAI, ICLR, ICML, NeurIPS, KDD, CVPR, S\&P, NDSS
	\item ECAI, ACML, ECML/PKDD, ICDM, SDM, CIKM, ESORICS, ACSAC
	\item PAKDD, KSEM, PRICAI, IJCNN
	\end{itemize}
	
	\item[Journals]<2->
	No more than two in each tier:
	\begin{itemize}
	\item TIFS, PAMI, TPDS, AIJ, MLJ, JMLR, JAIR
	\item TKDE, TFS, TII, TNNLS, TC, PR
	\item EWSA, KAIS, FGCS
	\end{itemize}	
	\end{description}

\item<3->
Read some recent papers in the selected venues,
and be familiar with their writing \emph{style}, 
\emph{length} and paper \emph{structure}.
\end{itemize}
\end{proof}
}

\onslide*{4-}{
\begin{proof}[Notes]
\begin{itemize}
\item<4-> 
Never ever \emph{double submission}!
	\begin{itemize}
	\item<5->
	\emph{Double submission} may lead to \emph{double publication},
	and it is \emph{unethical}.
	
	\item<6->
	The same idea should not be published twice in journals.
	\end{itemize}
	
\item<7->
Research work published in conferences,
can be extended for journals.
\begin{itemize}
\item<8->
Typically the conference paper needs to be extended for \SI{30}{\percent}.
\end{itemize}

\item<9->
\faMagic { } \textsc{TULIP-Lab} suggested practise:
\begin{itemize}
\item<10->
Complete the full draft, 
and shrink down \SI{30}{\percent} for conference submission;

\item<11->
Once accepted,
submit the full version to journal.
\end{itemize}
\end{itemize}
\end{proof}
}

\end{slide}
%%
%=================================================================
\begin{note}
	TBA
\end{note}
%%
%=================================================================


\section{Method}

%=================================================================
%%  
\begin{slide}%[toc=,bm=]
	{Non-Private SGD}	
		\begin{tikzpicture}[transform shape, rotate=0]
		\node [flipbox] (box) {%
			\begin{minipage}[t!]{\textwidth} 
%			\footnotesize 
				\begin{algorithm}[H]
				  	\SetKwProg{Fn}{function}{\{}{\}}
				 	\SetKwFunction{SGD}{StochasticGradientDescent}%
				 	\SetKwFunction{UNI}{Uniform}%

				\Fn(\tcp*[f]{The \emph{Stochastic Gradient Descent} Optimizer})
				{\SGD{$D = \{\vec{x}, y\}$}}
				{
 				    \KwIn{database $D$, $\epsilon$, $\delta$,
 				    and the loss function $L_{D,f}(h)$.}
					\KwOut{$\omega^*$}
					
					$\omega_0 = 0$ \;
					\For{$i \leftarrow 1$ \KwTo $T$}{
					$i_t \sim $ \UNI{$1, \cdots, n$}
					\tcp*[f]{select a random data example}\;
					$g_t = \bigtriangledown 
						l(\omega_{t-1}, (\vec{x}_{i_t}, y_{i_t})) 
						+ \lambda\bigtriangledown R(\omega_{t-1})$ \;
					$\omega_{t} = \prod_{\omega}(\omega_{t-1} - \eta_t g_t)$\;
					\tcp*[f]{projection onto the convex feasible set $\omega$}\;
					}
					
					\KwRet{$\omega^* = \omega_{T}$\;}					
				} 
					\caption{The \emph{Stochastic Gradient Descent} Optimizer}
				\end{algorithm}
		\end{minipage}
		};
		\node[fancytitle, rounded corners, right=10pt] at (box.north west) {\faLaptop};
		%\node[fancytitle, rounded corners] at (box.east) {$\clubsuit$};
		\end{tikzpicture} 	
\end{slide}
%%
%=================================================================
\begin{note}
	TBA
\end{note}
%%
%=================================================================


\section{Theoretical Analysis}

\section{Experiment Results}

%=================================================================
%%  
\begin{slide}%[toc=,bm=]
    {Privacy by K-Anonymous}
    \twotonebox{\faHandORight}{\parbox{.96\textwidth}
        {
            \begin{description}
                \item[K-Anonymity] 
                $4$-anonymity + $6$-anonymity $\nRightarrow$ $k$-anonymity, for any $k$
                \item[Task]
                \emph{Alex} is $28$ and he visited both hospitals
            \end{description}
        }
    }
    \onslide*{1-}{
        \centering \hfill \vspace*{1\baselineskip}
        
        \twocolumn[
        lcolwidth=0.5\linewidth,
        rcolwidth=0.5\linewidth
        ]
        {
            \begin{table}
                \fontsize{10pt}{10pt}\selectfont
                \setlength{\abovecaptionskip}{0pt}
                \setlength{\belowcaptionskip}{12pt}
                \centering
                \caption{Hospital A}
                \begin{tabular}{c|c|c|c}	
                    \toprule	
                    Zip  	&  	\textbf{Age}& 	\textbf{Nationality} 	& 	\textbf{Disease} 	\\
                    \midrule

\onslide*{2-}{\textcolor{orange}{130**}}\onslide*{1}{130**}
&   \onslide*{2-}{\textcolor{orange}{<30}}\onslide*{1}{<30}               
&   \onslide*{2-}{\textcolor{orange}{*}}\onslide*{1}{*}               
&   \onslide*{2-}{\textcolor{orange}{\rnode{d1}{AIDS}}}\onslide*{1}{AIDS}             
 \\
                    130** & <30 & * & Heart Disease \\
                    130** & <30 & * & Viral Infection \\
                    130** & <30 & * & Viral Infection \\
                    
                    \midrule

                    130** & 3*  & * & Cancer \\
                    130** & 3*  & * & Cancer \\
                    130** & 3*  & * & Cancer \\
                    130** & 3*  & * & Cancer \\
                    
                    \midrule
                    
                    130** & $\geq 40$ & * & Cancer \\
                    130** & $\geq 40$ & * & Heart Disease \\
                    130** & $\geq 40$ & * & Viral Infection \\
                    130** & $\geq 40$ & * & Viral Infection \\
        							
                    \bottomrule
                    
                \end{tabular}
            \end{table}
        } % left pane
        {	
            \begin{table}
    \fontsize{10pt}{10pt}\selectfont
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{12pt}
    \centering
    \caption{Hospital B}
    \begin{tabular}{c|c|c|c}	
        \toprule	
        Zip  	&  	\textbf{Age}& 	\textbf{Nationality} 	& 	\textbf{Disease} 	\\
        \midrule
        
\onslide*{2-}{\textcolor{orange}{\rnode{d2}{130**}}}\onslide*{1}{{130**} }
&   \onslide*{2-}{\textcolor{orange}{<35}}\onslide*{1}{<35}               
&   \onslide*{2-}{\textcolor{orange}{*}}\onslide*{1}{*}               
&   \onslide*{2-}{\textcolor{orange}{AIDS}}\onslide*{1}{AIDS}               
\\
        130** & <35 & * & Tuberculosis \\
        130** & <35 & * & Flu \\
        130** & <35 & * & Tuberculosis \\
        130** & <35 & * & Cancer \\
        130** & <35 & * & AIDS \\
        
        \midrule
        
        130** & $\geq 35$ & * & Cancer \\
        130** & $\geq 35$ & * & Cancer \\
        130** & $\geq 35$ & * & Cancer \\
        130** & $\geq 35$ & * & Tuberculosis \\
        130** & $\geq 35$ & * & Viral Infection \\
        130** & $\geq 35$ & * & Viral Infection \\
        
        \bottomrule
        
    \end{tabular}
\end{table}

			 \onslide*{3}{
    \psset{arrowscale=2,arrows=->}
    \nccurve[linecolor=red,angleA=0,angleB=160]{d1}{d2} 
}
      } % right pane	
    } % slides
\end{slide}
%%  
%=================================================================


\section{Conclusion}

%=================================================================
%%  
\begin{slide}%[toc=,bm=]
{\textsc{TULIP-Lab} Practise of Academic Writing }

    \smartdiagramset{description title width=2.2cm,
        description text width=12cm,
        %     module minimum height=.6cm
    }
    
    \centering
    
    \smartdiagram[priority descriptive diagram]{
        \faGithubAlt { } Git \emph{Private} Repository:  
        			\texttt{code} - \texttt{data} - \texttt{report},
        \faSlideshare { } Slides: Presentation \& Discussion,
        \faLaptop { } Empirical Design and \emph{Launch} the Research,
        \faPencilSquareO { } Full Report \emph{Writing},
        \faCheckSquareO { } Plagiarism \emph{Checking},
        \faSendO { } \emph{Submission}: \num{2} weeks prior to deadline
    } % Smart Diagram

\end{slide}
%%
%=================================================================
\begin{note}
	TBA
\end{note}
%%
%=================================================================



==> tex/mod-title.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% title
%%% TODO: Customize to your Own Title, Name, Address
%%%
\title{
%\textsc{\small{Fundamentals of Learning and Information Processing}}
%\\ \textsc{\Large{Session \sessionNumber: \sessionTitle}}}
\textsc{\Large{\sessionTitle}}}
\author{%Multi authors
    \parbox{4cm}{%
        \centering 
        \begin{tikzpicture}
            \clip (0,0) circle (.066\textwidth); %2cm
            \node[anchor=center] at (0,0) %(0.62,-3) 
            {\includegraphics[width=0.136\textwidth]{./graphics/tulip/gangli.eps}};
        \end{tikzpicture}
       \\ \centering Gang Li %\\CSRI, SIT
    } %parbox
%    \hspace{1cm}
%    \parbox{4cm}{%
%        \centering 
%        \begin{tikzpicture}
%            \clip (0,0) circle (.066\textwidth); %2cm
%            \node[anchor=center] at (0,0) %(0.62,-3) 
%            {\includegraphics[width=0.136\textwidth]{figures/tulip/gangli.eps}};
%        \end{tikzpicture}
%       \\ \centering Gang Li %\\CSRI, SIT
%    } %parbox
%\vspace{.25cm}
%\\Center for Cyber Security Research and Innovation
\vspace{.25cm}
\\Deakin University, Australia
% \and % more authors
}
\date{\gitCommitterDate}


% Customize the setting of slides
\pdsetup{
% TODO: Customize the left footer, and right footer
%lf=\href{http://www.tulip.org.au}{\copyright 2015 \textsc{TULIP Lab (G. Li)}},
cf={\textsc{TULIP Lab: \sessionTitle}},
rf=\href{http://www.tulip.org.au}{
%Last Changed by: \textsc{\gitCommitterName}\ 
\gitVtagn-\gitAbbrevHash\ (\gitAuthorDate)
},
%trans=Fade,
list={labelsep=1em,leftmargin=*,itemsep=0pt,topsep=5pt,parsep=0pt},
}

\hypersetup{
  pdftitle={\sessionTitle},
  pdfauthor={Gang Li},
  pdfpagemode={FullScreen},
  pdfborder={0 0 0}
}


